Witches' Brew: Industrial Scale Data Poisoning via Gradient Matching

Data Poisoning attacks modify training data to maliciously control a model trained on such data. In this work, we focus on targeted poisoning attacks which cause a reclassification of an unmodified test image and as such breach model integrity. We consider a particularly malicious poisoning attack that is both "from scratch" and "clean label", meaning we analyze an attack that successfully works against new, randomly initialized models, and is nearly imperceptible to humans, all while perturbing only a small fraction of the training data. Previous poisoning attacks against deep neural networks in this setting have been limited in scope and success, working only in simplified settings or being prohibitively expensive for large datasets. The central mechanism of the new attack is matching the gradient direction of malicious examples. We analyze why this works, supplement with practical considerations. and show its threat to real-world practitioners, finding that it is the first poisoning method to cause targeted misclassification in modern deep networks trained from scratch on a full-sized, poisoned ImageNet dataset. Finally we demonstrate the limitations of existing defensive strategies against such an attack, concluding that data poisoning is a credible threat, even for large-scale deep learning systems.

==> plots/bilevel.tex <==
\section{Relation to bilevel-optimization-based data poisoning}

\subsection{Approximations to Bi-level optimization}
To understand the difference between our \textit{blind passengers} approach and MetaPoison \cite{huang_metapoison:_2020}, it is instructive to compare the gradient w.r.t. to the poisoned data for both loss terms in the case of a single unrolling step of MetaPoison and taking the normalization of the cosine as one. The gradient for \cref{eq:bp_loss} in this setting can be written informally as the matrix product: 
\begin{equation}
     \nabla_x \nabla_\theta \mathcal{L}(x_p, y_p, \theta) \cdot \nabla_\theta \mathcal{L}(x_t, y_t, \theta) 
\end{equation}
for some parameter vector $\theta$,
whereas the gradient of the MetaPoison objective $\mathcal{L}(x_t, y_t, \theta - \tau\nabla_\theta \mathcal{L}(x_p, y_p, \theta))$ for $\theta$ (note that MetaPoison also updates from the "clean" $\theta$) is given by
\begin{equation}
    \nabla_x \nabla_\theta \mathcal{L}(x_p, y_p, \theta) \cdot \nabla_\theta \mathcal{L}\left(x_t, y_t, \theta - \tau\nabla_\theta(x_p, y_p, \theta)\right) 
\end{equation}
Interestingly, both gradients are structurally very similar, differing only at the parameter location, where the gradient w.r.t to the target is computed. If we assume the gradient at $\theta$ to be similar to the gradient at $\theta - \tau\nabla_\theta \mathcal{L}$, as given at the end of training, where we draw $\theta$ for the \textit{blind-passengers} approach, then this yields a good approximation to the MetaPoison objective.

In terms of approximating the bilevel objective, the proposed objective is a first step of the iterative method discussed in \cite{geiping_parametric_2019-2} \jg{...., is this an iterated majorizer of contrastive loss?}

For further comparison, recall the bi-level optimization poisoning setup :

\begin{equation*}
    \min_{x_p} \mathcal{L} \left( x_t, y_t, \theta(x_p) \right) \st \theta(x_p) \in \argmin_\theta \mathcal{L}(x_p, y_p, \theta).
\end{equation*}

If we assume that the minimizer $\theta(x_p)$ satisfies the condition that $\nabla_\theta \mathcal{L}(x_p, y_p, \theta) = 0$. Then, by chain rule, and implicit function theorem (assuming the hessian $H_\theta(\mathcal{L})(x_p, y_p, \theta)$ is invertible), we have that the gradient of the full bilevel optimization problem can be written as 
\begin{equation}
    \nabla_x \mathcal{L}(x_t, y_t, \theta) - \nabla_x \nabla_\theta \mathcal{L}(x_p, y_p, \theta) \cdot (\nabla^2_\theta \mathcal{L}(x_p, y_p, \theta))^{-1} \nabla_\theta \mathcal{L}(x_t, y_t, \theta)
\end{equation}
 \cite{munoz-gonzalez_towards_2017,demontis_why_2019}. Noting that the first term is a constant, we again find this term closely related to the proposed setting, only the last term in the product is preconditioned by the curvature of the loss landscape.
This also related to \cite{koh_understanding_2017}.

